Obaleth: Build Your Own GPU Communication Stack

Machine learning systems specialize computation to the workload and hardware, but communication remains in generic libraries whose device code and transport decisions are not visible to high-level compilers. We present Obaleth, a compiler that makes GPU-initiated communication part of a kernel's intermediate representation, co-optimizes it alongside computation, and lowers it to specialized transport code. Obaleth plans completions around buffer lifetimes and optimizes memory ordering, synchronization, and batching across NVIDIA and AMD GPUs. On H100 GPUs, Obaleth sends small messages up to 3.3$\times$ faster, and on 256 GPUs runs all-to-all 1.25$\times$ and 2.3$\times$ faster than NVSHMEM and NCCL GIN, with much smaller memory and register use. In vLLM, it serves Qwen3-235B on 16 B200 GPUs and answers requests up to 1.29$\times$ faster than with DeepEP.

==> code-designs.tex <==
\iflatexml\else
\RequirePackage{tcolorbox}
\tcbuselibrary{skins}
\fi
\makeatletter

\definecolor{cdGrey}{HTML}{ECEEF1}
\definecolor{cdBlue}{HTML}{DCE7F8}
\definecolor{cdAmber}{HTML}{FCEDC2}
\definecolor{cdRule}{HTML}{AEB5C0}
\definecolor{cdInk}{HTML}{1D6F64}

\newcommand{\cd@small}{\fontsize{\fpeval{0.92*\f@size}}{\f@baselineskip}\selectfont}
\newcommand{\cd@strut}{\rule[-0.24em]{0pt}{0.98em}}

\newcommand{\cd@square}[3]{%
  {\setlength{\fboxsep}{0pt}%
   \colorbox{#1}{\cd@strut\kern#2\cd@small#3\kern#2}}}

\iflatexml
\newcommand{\cd@pill}[2][]{\colorbox{cdGrey}{#2}}
\else
\newtcbox{\cd@pill}[1][]{on line, enhanced jigsaw,
  colback=cdGrey, colframe=cdGrey, boxrule=0pt, arc=1.8pt,
  left=1.8pt, right=1.8pt, top=0pt, bottom=0pt, boxsep=0pt,
  before upper={\cd@strut\cd@small}, #1}
\fi

\expandafter\def\csname cd@style@0\endcsname#1{#1}
\expandafter\def\csname cd@style@1\endcsname#1{\cd@square{cdGrey}{1.4pt}{#1}}
\expandafter\def\csname cd@style@2\endcsname#1{\cd@pill{#1}}
\expandafter\def\csname cd@style@3\endcsname#1{%
  \cd@pill[colback=cdBlue, colframe=cdBlue]{#1}}
\expandafter\def\csname cd@style@4\endcsname#1{\cd@square{cdAmber}{1.4pt}{#1}}
\expandafter\def\csname cd@style@5\endcsname#1{%
  \cd@pill[colback=white, colframe=cdRule, boxrule=0.4pt,
           left=1.4pt, right=1.4pt]{#1}}
\expandafter\def\csname cd@style@6\endcsname#1{\textcolor{cdInk}{#1}}

\ExplSyntaxOn
\cs_generate_variant:Nn \tl_replace_all:Nnn { NV }
\tl_const:Nx \c__cd_underscore_tl { \char_generate:nn { `_ } { 8 } }
\cs_new_protected:Npn \__cd_typeset:n #1 { \codestyle { \texttt { #1 } } }
\cs_new_protected:Npn \__cd_typeset_op:n #1 { \opstyle { \texttt { #1 } } }
\cs_new_protected:Npn \__cd_underscores:N #1
{
  \tl_replace_all:NVn #1 \c__cd_underscore_tl
    { \char 95 \scan_stop: }
}
\NewDocumentCommand{\code}{m}
{
  \tl_set:Nn \l_tmpa_tl { #1 }
  \__cd_underscores:N \l_tmpa_tl
  \exp_args:NV \__cd_typeset:n \l_tmpa_tl
}
\NewDocumentCommand{\op}{m}
{
  \tl_set:Nn \l_tmpa_tl { #1 }
  \__cd_underscores:N \l_tmpa_tl
  \exp_args:NV \__cd_typeset_op:n \l_tmpa_tl
}
\ExplSyntaxOff

\providecolor{abMark}{HTML}{FBE3A0}
\newcommand{\opstyle}[1]{\cd@pill[colback=cdGrey, colframe=cdGrey]{\bfseries#1}}

\let\codestyle\@firstofone
\newcommand{\UseCodeStyle}[1]{%
  \@ifundefined{cd@style@#1}{%
    \PackageError{code-designs}{Unknown code style `#1'}%
      {Use a number from 0 to 6.}}{%
    \expandafter\let\expandafter\codestyle\csname cd@style@#1\endcsname}}

\makeatother


==> listing-designs.tex <==
\makeatletter

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{commentgray}{gray}{0.45}
\definecolor{abNavy}{HTML}{1F3A6B}
\definecolor{abBlue}{HTML}{2457A6}
\definecolor{abTeal}{HTML}{1D6F64}
\definecolor{abBrick}{HTML}{9C3B26}
\definecolor{abGray}{HTML}{6B7280}
\definecolor{abRule}{HTML}{B8BEC8}
\definecolor{abPanel}{HTML}{F2F4F7}
\definecolor{abAccent}{HTML}{3B6EA8}
\definecolor{abMark}{HTML}{FBE3A0}

\def\lst@makecaption{\def\@captype{lstlisting}\ld@lstcaption}
\long\def\ld@lstcaption#1#2{%
  \@makecaption{#1}{#2}%
\ifdim\belowcaptionskip=\z@\else\vskip\belowcaptionskip\fi}

\lstdefinelanguage{mlir}{
  morekeywords={func,return,constant},
  sensitive=true,
  morecomment=[l]{//},
}
\lstdefinestyle{lang-cuda}{
  language=C++,
  morekeywords={__global__,__device__},
  morekeywords=[2]{uint32_t,uint64_t,DeviceContext,RemoteRegion,LocalRegion},
}
\lstdefinestyle{lang-py}{
  language=Python,
  morekeywords={None},
}
\lstdefinestyle{lang-mlir}{
  language=mlir,
}

\newcommand{\ld@langs}[1]{%
  \lstdefinestyle{#1-cuda}{style=#1, style=lang-cuda}%
  \lstdefinestyle{#1-py}{style=#1, style=lang-py}%
  \lstdefinestyle{#1-mlir}{style=#1, style=lang-mlir}%
\lstdefinestyle{#1-default}{style=#1}}

\lstdefinestyle{ld-common}{
  basicstyle=\ttfamily\fontsize{7}{8}\selectfont,
  columns=fullflexible,
  keepspaces=true,
  showstringspaces=false,
  tabsize=2,
  breaklines=false,
  numbers=none,
  belowcaptionskip=0pt,
}

\lstdefinestyle{cppstyle}{
  language=C++,
  backgroundcolor=\color{backcolour},
  commentstyle=\color{commentgray},
  keywordstyle=\color{magenta},
  numberstyle=\tiny\color{codegray},
  stringstyle=\color{codepurple},
  basicstyle=\ttfamily\footnotesize,
  breakatwhitespace=false,
  breaklines=true,
  captionpos=b,
  keepspaces=true,
  numbers=left,
  numbersep=5pt,
  showspaces=false,
  showstringspaces=false,
  showtabs=false,
  tabsize=2,
  belowcaptionskip=0pt,
}
\lstdefinestyle{base}{
  style=cppstyle,
  basicstyle=\ttfamily\scriptsize,
  numbers=none,
  breaklines=false,
}
\lstdefinestyle{base-cuda}{
  style=base,
  language=C++,
  morekeywords={__global__,__device__,uint32_t,uint64_t},
}
\lstdefinestyle{base-py}{
  style=base,
  language=Python,
  morekeywords={tl,triton},
}
\lstdefinestyle{base-mlir}{
  style=base,
  language=mlir,
}
\lstdefinestyle{base-default}{style=cppstyle}
\def\ld@font@base{pcr}

\lstdefinestyle{A}{
  style=ld-common,
  frame=tb,
  framerule=0.6pt,
  rulecolor=\color{black},
  framesep=3pt,
  keywordstyle=\bfseries\color{abNavy},
  keywordstyle=[2]\color{abTeal},
  commentstyle=\color{abGray},
  stringstyle=\color{abBrick},
  captionpos=t,
  belowcaptionskip=6pt,
}
\ld@langs{A}
\def\ld@font@A{zi4}

\lstdefinestyle{B}{
  style=ld-common,
  backgroundcolor=\color{abPanel},
  frame=l,
  framerule=1.6pt,
  rulecolor=\color{abAccent},
  framesep=5pt,
  xleftmargin=6.6pt,
  framextopmargin=2pt,
  framexbottommargin=2pt,
  keywordstyle=\color{abBlue},
  keywordstyle=[2]\color{abTeal},
  commentstyle=\color{abGray},
  stringstyle=\color{abBrick},
  captionpos=b,
}
\ld@langs{B}
\def\ld@font@B{zi4}

\lstdefinestyle{C}{
  style=ld-common,
  numbers=left,
  numberstyle=\fontsize{5.5}{8.6}\selectfont\ttfamily\color{abGray},
  numbersep=7pt,
  frame=l,
  framerule=0.4pt,
  rulecolor=\color{abRule},
  framesep=5pt,
  xleftmargin=15pt,
  keywordstyle=\bfseries\color{abNavy},
  keywordstyle=[2]\color{abTeal},
  commentstyle=\color{abGray},
  stringstyle=\color{abBrick},
  captionpos=b,
}
\ld@langs{C}
\def\ld@font@C{zi4}

\lstdefinestyle{D}{
  style=ld-common,
  xleftmargin=1em,
  keywordstyle=\bfseries,
  keywordstyle=[2]{},
  commentstyle=\itshape\color{black!62},
  stringstyle={},
  captionpos=b,
}
\ld@langs{D}
\def\ld@font@D{ntxtt}

\newcommand{\ld@hl}[1]{%
  {\setlength{\fboxsep}{0.9pt}\kern-0.9pt%
  \colorbox{abMark}{\vphantom{(}\textbf{#1}}\kern-0.9pt}}
  \lstdefinestyle{E}{
    style=ld-common,
    frame=tb,
    framerule=0.6pt,
    rulecolor=\color{black},
    framesep=3pt,
    keywordstyle=\bfseries\color{black!80},
    keywordstyle=[2]{},
    commentstyle=\color{abGray},
    stringstyle={},
    emphstyle=\ld@hl,
    captionpos=t,
    belowcaptionskip=6pt,
  }
  \ld@langs{E}
  \lstdefinestyle{E-cuda}{
    style=E, style=lang-cuda,
    emph={put,put_inline,put_signal,signal,wait,wait_signal,quiet,drain},
  }
  \lstdefinestyle{E-py}{
    style=E, style=lang-py,
    alsoletter={.},
    emph={obaleth.endpoint,obaleth.put,obaleth.put_inline,obaleth.put_signal,
      obaleth.signal,obaleth.wait,obaleth.wait_signal,obaleth.quiet,
    obaleth.drain},
  }
  \def\ld@font@E{zi4}

  \lstdefinestyle{F-card}{
    style=ld-common,
    keywordstyle=\color{abBlue},
    keywordstyle=[2]\color{abTeal},
    commentstyle=\color{abGray},
    stringstyle=\color{abBrick},
    captionpos=b,
  }
  \lstdefinestyle{F}{
    style=F-card,
    frame=single,
    frameround=tttt,
    framerule=0.4pt,
    rulecolor=\color{abRule},
    framesep=3pt,
    xleftmargin=3.4pt,
    xrightmargin=3.4pt,
  }
  \ld@langs{F}
  \def\ld@font@F{zi4}
  \newcommand{\ld@setupcard}{%
    \RequirePackage{tcolorbox}%
    \tcbuselibrary{most}%
    \tcbset{
      ldcard/.style={
        enhanced, listing only,
        colback=white, colframe=abRule, boxrule=0.4pt, arc=2pt,
        left=4pt, right=2pt, top=2pt, bottom=2pt, boxsep=0pt,
        colbacktitle=abPanel, coltitle=abGray,
        fonttitle=\fontsize{6.5}{7.5}\selectfont\sffamily,
        toptitle=1.5pt, bottomtitle=1.5pt, titlerule=0.4pt,
        before skip=2pt, after skip=0pt,
      },
    }%
    \newtcblisting{codecard}[2]{ldcard, title={##2},
      listing options={style=F-card, style=lang-##1,
    aboveskip=0pt, belowskip=0pt}}%
  }
  \newcommand{\cardcaption}[1]{%
  \refstepcounter{lstlisting}\@makecaption{\lstlistingname~\thelstlisting}{#1}}

  \let\listingnote\@empty
  \def\ld@F{F}
  \newcommand{\UseListingDesign}[1]{%
    \@ifundefined{ld@font@#1}{%
      \PackageError{listing-designs}{Unknown listing design `#1'}%
    {Use one of: base, A, B, C, D, E, F.}}{}%
    \lstdefinestyle{cudastyle}{style=#1-cuda}%
    \lstdefinestyle{pystyle}{style=#1-py}%
    \lstdefinestyle{mlirstyle}{style=#1-mlir}%
    \lstset{style=#1-default}%
    \edef\ttdefault{\csname ld@font@#1\endcsname}%
    \@ifundefined{ld@note@#1}%
    {\let\listingnote\@empty}%
    {\expandafter\let\expandafter\listingnote\csname ld@note@#1\endcsname}%
    \def\ld@arg{#1}%
    \ifx\ld@arg\ld@F\expandafter\ld@setupcard\fi
  }

  \makeatother

